How a General-Purpose Commonsense Ontology can Improve Performance of Learning-Based Image Retrieval

The knowledge representation community has built general-purpose ontologies which contain large amounts of commonsense knowledge over relevant aspects of the world, including useful visual information, e.g.: "a ball is used by a football player", "a tennis player is located at a tennis court". Current state-of-the-art approaches for visual recognition do not exploit these rule-based knowledge sources. Instead, they learn recognition models directly from training examples. In this paper, we study how general-purpose ontologies---specifically, MIT's ConceptNet ontology---can improve the performance of state-of-the-art vision systems. As a testbed, we tackle the problem of sentence-based image retrieval. Our retrieval approach incorporates knowledge from ConceptNet on top of a large pool of object detectors derived from a deep learning technique. In our experiments, we show that ConceptNet can improve performance on a common benchmark dataset. Key to our performance is the use of the ESPGAME dataset to select visually relevant relations from ConceptNet. Consequently, a main conclusion of this work is that general-purpose commonsense ontologies improve performance on visual reasoning tasks when properly filtered to select meaningful visual relations.

==> ex/ex1.tex <==
\includegraphics[width=3cm,height=2cm,keepaspectratio]{./img/1.jpg}
 
1) \textcolor{red}{Seamen} inside a \textcolor{red}{navy} \textcolor{red}{vessel} \textcolor{red}{communicate} over the \textcolor{red}{radio}. 
& 
\setlength{\tabcolsep}{6pt}
\begin{tabular}{ >{\centering}m{2cm}<{\centering} m{2cm} m{2cm} m{2cm} m{2cm} m{2cm} }
MIL\_STEM Pos: 5000 &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/1_1b.jpg} & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/1_2b.jpg} & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/1_3b.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/1_4b.jpg} \\
\hline
CN\_MAX Pos: \textbf{15} & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/1_1.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/1_2.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/1_3.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/1_4.jpg} \\
\end{tabular}

==> ex/ex4.tex <==
\includegraphics[width=3cm,height=2.5cm,keepaspectratio]{./img/4.jpg}

4) \textcolor{blue}{People} \textcolor{blue}{stand} near a \textcolor{blue}{large} \textcolor{blue}{modern} \textcolor{red}{art} \textcolor{red}{sculpture}.
& 
\setlength{\tabcolsep}{6pt}
\begin{tabular}{ >{\centering}m{2cm}<{\centering} m{2cm} m{2cm} m{2cm} m{2cm} m{2cm} }
MIL\_STEM Pos: 149 &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/4_1b.jpg} & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/4_2b.jpg} & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/4_3b.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/4_4b.jpg} \\
\hline
CN\_MAX Pos: \textbf{1} & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/4_1.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/4_2.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/4_3.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/4_4.jpg} \\
\end{tabular}

==> ex/ex5.tex <==
\includegraphics[width=3cm,height=2cm,keepaspectratio]{./img/5.jpg}

\textcolor{red}{Folded} \textcolor{blue}{glasses} \textcolor{blue}{sit} \textcolor{blue}{next} to a \textcolor{blue}{filled} \textcolor{blue}{black}-and-\textcolor{blue}{white} \textcolor{red}{patterned} \textcolor{red}{mug} with a \textcolor{red}{buried} \textcolor{red}{utensil}.

& 
\setlength{\tabcolsep}{6pt}
\begin{tabular}{ >{\centering}m{2cm}<{\centering} m{2cm} m{2cm} m{2cm} m{2cm} m{2cm} }
MIL\_STEM Pos: 122 &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/5_1b.jpg} & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/5_2b.jpg} & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/5_3b.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/5_4b.jpg} \\
\hline
CN\_MAX Pos: \textbf{16} & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/5_1.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/5_2.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/5_3.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/5_4.jpg} \\
\end{tabular}

==> ex/ex7.tex <==

\includegraphics[width=3cm,height=2.5cm,keepaspectratio]{./img/7.jpg}

6) Here \textcolor{blue}{is} a \textcolor{red}{soul} in the \textcolor{blue}{image} alone.
& 
\setlength{\tabcolsep}{6pt}
\begin{tabular}{ >{\centering}m{2cm}<{\centering} m{2cm} m{2cm} m{2cm} m{2cm} m{2cm} }
MIL\_STEM Pos: \textbf{1831} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/7_1b.jpg} & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/7_2b.jpg} & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/7_3b.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/7_4b.jpg} \\
\hline
CN\_MAX Pos: 2602 & 
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/7_1.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/7_2.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/7_3.jpg} &
\includegraphics[width=2cm,height=1.5cm,keepaspectratio]{./img/7_4.jpg} \\
\end{tabular}

==> sections/acknowledgments.tex <==
\section*{Acknowledgments}

This work was partially funded by grant FONDECYT 1151018.

==> sections/future_works.tex <==
\section{Future Works}

This paper proposed a methodology to detect words in images without training an specific word detector. For this, we use the common sense knowledge present in ConceptNet, powered by the visual knowledge present on ESPGAMES. Even though the good results of this approach, we are not using the whole ConceptNet's potential. In fact, we are not using either the types of relationships or distances greater than 1 in ConceptNet. As future works, we believe those components are key to continue improving the performance. 

Another open problem is how to solve the polysemy and synonymy issues presents on ConceptNet. In ConceptNet the node \textit{fly} has relations regarding to the \textit{verb fly} and to the \textit{insect fly}, meanwhile \textit{computer} has relations that \textit{pc} does not. Moreover, the stemming process increases the ambiguity transforming \textit{bowling} in \textit{bowl}. This are well known ConceptNet problems, and some works have been done in this area (for text mining) [\textbf{??}]. 

Finally, regarding image retrieval, future works could explore tree improvement to our approach. First, we could use the spatial information of the words detection. Currently, to detect \textit{tuxedo}, we look for images with high detections of \textit{jacket}, \textit{black}, etc, but we are not constraining them to fire in the same location. Second, the sentence understanding is key. Examples such as "\textit{a road without cars}" produce really bad image retrieval responses. Finally, our score is a plane multiplication of the detectors outputs but, empirically, we have seen that query sentences usually have words that are more important to detect than others. Future works could try adding weight to our score.

